A clustering aggregation algorithm on neutral-atoms and annealing quantum processors

This work presents a hybrid quantum-classical algorithm to perform clustering aggregation, designed for neutral-atoms quantum computers and quantum annealers. Clustering aggregation is a technique that mitigates the weaknesses of clustering algorithms, an important class of data science methods for partitioning datasets, and is widely employed in many real-world applications. By expressing the clustering aggregation problem instances as a Maximum Independent Set (MIS) problem and as a Quadratic Unconstrained Binary Optimization (QUBO) problem, it was possible to solve them by leveraging the potential of Pasqal's Fresnel (neutral-atoms processor) and D-Wave's Advantage QPU (quantum annealer). Additionally, the designed clustering aggregation algorithm was first validated on a Fresnel emulator based on QuTiP and later on an emulator of the same machine based on tensor networks, provided by Pasqal. The results revealed technical limitations, such as the difficulty of adding additional constraints on the employed neutral-atoms platform and the need for better metrics to measure the quality of the produced clusterings. However, this work represents a step towards a benchmark to compare two different machines: a quantum annealer and a neutral-atom quantum computer. Moreover, findings suggest promising potential for future advancements in hybrid quantum-classical pipelines, although further improvements are needed in both quantum and classical components.

==> results.tex <==
\section{Results}

\subsection{Metrics}

\subsubsection{Time} An important detail to consider when comparing the efficiency of machines is the total time necessary to execute the algorithm. Due to the inherent differences of the quantum platforms used to perform the experiments, defining how to measure the execution time is not obvious, and requires a more thorough discussion.

The processing cycle for Pasqal's Fresnel, shown in Figure \ref{fig:fresnel_qpu_processing}, is made up of the following steps: register loading, sub-register rearranging, and quantum processing. Unfortunately, at the moment the only disclosed information regarding timing is that the quantum processing step in a processing cycle takes at most $100 \mu s$. Such information concerning the time execution on the Fresnel QPU has been provided by the Pasqal Team via private communication.

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/experiments/QPU_Processing_Cycle_Steps-1.png}
    \caption{Steps of the QPU processing; at the moment, only quantum processing time has been disclosed, with a maximum value of $100 \mu s$.}
    \label{fig:fresnel_qpu_processing}
\end{figure}

On D-Wave's Advantage QPU, the time necessary to actually execute a job (in this context known as QMI, or Quantum Machine Instruction) is referred to as \emph{access time}, which does not take in account the time necessary for data to go back and forth to the cloud, or for the QMI to wait in queue for the QPU, but only the time effectively used by the QPU to solve the problem. Access time can be further broken up in several phases, as shown in Figure \ref{fig:dwave_access_time} \cite{dwavesysOperationTiming}, namely programming time, necessary to embed the problem onto the machine, plus sampling time, which is the time required to execute the algorithm and read results. In order to compare similar phases with Fresnel, the only time information taken in consideration will be the sampling time.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/experiments/access_time.png}
    \caption{Detail of phases in QPU access time for D-Wave's Advantage QPU. Figure is taken from \cite{dwavesysOperationTiming}.}
    \label{fig:dwave_access_time}
\end{figure}

For the emulated version of Fresnel on QuTip, the execution time was obtained by calling Python's function \texttt{time.time()}, which returns the current UTC time, before and after the execution of the quantum simulation; execution time was then computed by taking the difference between the two timestamps.

For the emulated version of Fresnel on tensor networks, which runs in the Pasqal's cloud infrastructure, the time information is provided in the results.

\subsubsection{Number of returned clusters}
% \gbnote{numero di clusters ritornati}
The metric chosen to evaluate the quality of solutions is the probability of returning a solution with a certain number of clusters; in particular, a good algorithm should return the correct number of clusters (i.e. the size of the MWIS) with the highest probability.


\subsection{Results comparison}

A comparison of the execution times on the different platforms is shown in Table \ref{tab:time_comparisons}. It is possible to observe how the times of experiments run on real quantum hardware have comparable orders of magnitude (with the experiment on Advantage QPU without silhouette constraint being slightly faster, in the order of $10^{4} \mu s$, than the other two, in the order of $10^{5} \mu s$).

\begin{table}[ht!]
    \centering
    \begin{tabular}{||l|c||}
        \hline
        \textbf{Platform} & \textbf{Total time} \\ 
        \hline 
        Fresnel (TN emulator) & $1.3 \cdot 10^{5} \mu s$ \\ 
        \hline 
        Fresnel & $1.00 \cdot 10^{5} \mu s$ \\
        \hline 
        Advantage QPU (without silhouette) & $8.82 \cdot 10^{4} \mu s$ \\
        \hline 
        Advantage QPU (with silhouette) & $1,30 \cdot 10^{5} \mu s$ \\
        \hline 
    \end{tabular}
    \caption{Comparison of the execution times for the clustering aggregation algorithms on the different quantum platforms.}
    \label{tab:time_comparisons}
\end{table}
Figure \ref{fig:occurrences_pasqal} shows the probabilities (in percentage) of reading a given bitstring from the output of the experiments on Fresnel (both emulated and real hardware), while Figure \ref{fig:occurrences_dwave} shows those related to both experiments on Advantage QPU.



\begin{figure}[ht!]
    \centering
    \subfigure[QuTiP emulated Fresnel.]{
        \includegraphics[width=0.9\linewidth]{figures/results/num_occurrences_emu.pdf}
    }

    \subfigure[Real hardware Fresnel.]{
        \includegraphics[width=0.9\linewidth]{figures/results/num_occurrences_fresnel.pdf}
    }
    \caption{Probability (in percentage) of reading a certain bistring after measuring the experiments on QuTiP emulated and real hardware Fresnel. (a) shows the 20 most likely bitstrings from the experiment on the emulator, while (b) the 20 most likely bitstrings from the real hardware experiment.}
    \label{fig:occurrences_pasqal}
\end{figure}

\begin{figure}[ht!]
    \centering
    \subfigure[Advantage QPU (without silhouette).]{
        \includegraphics[width=0.9\linewidth]{figures/results/num_occurrences_dwave.pdf}
    }

    \subfigure[Advantage QPU (with silhouette).]{
        \includegraphics[width=0.9\linewidth]{figures/results/num_occurrences_dwave_silhouette.pdf}
    }
    \caption{Probability (in percentage) of reading a certain bistring for the experiments on Advantage QPU, both without and with the silhouette constraint. (a) shows the 20 most likely bitstrings from the experiment that does not use the silhouette information, while (b) the 20 most likely bitstrings from the experiment that uses the silhouette information as a constraint.}
    \label{fig:occurrences_dwave}
\end{figure}


